"Wikily" Supervised Neural Translation Tailored to Cross-Lingual Tasks

We present a simple but effective approach for leveraging Wikipedia for neural machine translation as well as cross-lingual tasks of image captioning and dependency parsing without using any direct supervision from external parallel data or supervised models in the target language. We show that first sentences and titles of linked Wikipedia pages, as well as cross-lingual image captions, are strong signals for a seed parallel data to extract bilingual dictionaries and cross-lingual word embeddings for mining parallel text from Wikipedia. Our final model achieves high BLEU scores that are close to or sometimes higher than strong supervised baselines in low-resource languages; e.g. supervised BLEU of 4.0 versus 12.1 from our model in English-to-Kazakh. Moreover, we tailor our wikily supervised translation models to unsupervised image captioning, and cross-lingual dependency parser transfer. In image captioning, we train a multi-tasking machine translation and image captioning pipeline for Arabic and English from which the Arabic training data is a translated version of the English captioning data, using our wikily-supervised translation models. Our captioning results on Arabic are slightly better than that of its supervised model. In dependency parsing, we translate a large amount of monolingual text, and use it as artificial training data in an annotation projection framework. We show that our model outperforms recent work on cross-lingual transfer of dependency parsers.

==> alg.tex <==
\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LState{\State \algbackskip}%
\makeatother

\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LComment{\Comment \algbackskip}%
\makeatother

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\begin{figure}[t!]
\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\vspace{0.1cm}
%\noindent\rule{0.5\textwidth}{0.4pt}
\begin{algorithmic}[0]
\scriptsize
\LState {{\bf Definitions: }{ 1) $e$ is English, $f$ is the foreign language, and $g$ is a language similar to $f$}, 2) $\colorbox{red!30}{learn\_dict}(P)$ extracts a bilingual dictionary from parallel data $P$, 3) $\colorbox{orange!30}{t}(x| m)$ translates input $x$ given model $m$, , 4) $\colorbox{yellow!30}{pretrain}(x)$ pretrains on monolingual data $x$ using MASS~\protect\cite{song2019mass}, 5) $\colorbox{green!30}{train}(P | m)$ trains on parallel data $P$ initialized by model $m$, 6) $\colorbox{blue!10}{bt\_train}(x_1, x_2 | m)$ trains iterative back-translation on monolingual data $x_1 \in e$ and $x_2 \in f$ initialized by model $m$. }
 \LState {{\bf Inputs: }{ 1) Wikipedia documents $\docs^{(e)}$, $\docs^{(f)}$, and $\docs^{(g)}$}, 2) Monolingual word embedding vectors $\embed_e$ and $\embed_f$, 3) Set of linked pages from Wikipedia \colorbox{pink!30}{$\comp$}, their aligned titles $\titles$, and their first sentence pairs $\first$, 4) Set of paired image captions $\captions$, and 5) Gold-standard parallel data $\bitext^{(e,g)}$.}
\vspace{0.1cm}


\LState{\bf Algorithm:}
%~\\~~
\LState{\bf $\rightarrow$ Learn bilingual dictionary and embeddings}
\State $\seed = \first \cup \captions \cup \titles$ 
\State $\dict^{(f,e)} = \colorbox{red!30}{learn\_dict}(\seed)$
\State $\dict^{(g,e)} = \colorbox{red!30}{learn\_dict}(\bitext^{(e,g)})$ \Comment{\colorbox{gray!15}{Related language}}
\State Learn $\embed_e \rightarrow \embed'_e$ and $\embed_f\rightarrow \embed'_f$ using $\dict^{(f,e)} \cup \dict^{(g,e)}$
%~\\~~
\LState{\bf $\rightarrow$ Mine parallel data}
\State Extract comparable sentences ${\cal Z}$ from \colorbox{pink!30}{$\comp$}
\State Extract $\bitext^{(f,e)}$ from ${\cal Z}$.% using Eq.~\ref{eq1}. \Comment{\colorbox{gray!15}{Cosine sim.}}
\State $\bitext^{(f,e)} = \bitext^{(f,e)} \cup \titles$ \Comment{\colorbox{gray!15}{Mined Data}}
%~\\~~
\LState{\bf $\rightarrow$ Train MT with pretraining and back-translation}
\State $\theta_0= \colorbox{yellow!30}{pretrain}(\docs^{(e)} \cup \docs^{(f)} \cup \docs^{(g)})$ \Comment{\colorbox{gray!15}{MASS Training}}
\State $\theta_{\rightleftarrows} = \colorbox{green!30}{train}(\bitext^{(f,e)} \cup \bitext^{(g,e)} | \theta_0 )$ \Comment{\colorbox{gray!15}{NMT Training}}
\State $\bitext^{(e\rightarrow f)} = (\colorbox{orange!30}{t}(\docs^{(f)} | \theta_{\rightleftarrows}),\docs^{(f)})$
\State $\bitext^{(f\rightarrow e)} = (\colorbox{orange!30}{t}(\docs^{(e)} | \theta_{\rightleftarrows}),\docs^{(e)})$
\State  $\bitext'^{(f,e)} = \bitext^{(e\rightarrow f)} \cup \bitext^{(f\rightarrow e)} \cup \bitext^{(f,e)}$
\State $\theta'_{\rightleftarrows}= \colorbox{green!30}{train}(\bitext'^{(f,e)} | \theta_0)$
\State  $\theta*_{\rightleftarrows}= \colorbox{blue!10}{bt\_train}(\docs^{(e)}, \docs^{(f)}|\theta'_{\rightleftarrows})$
%~\\~~
\LState {{\bf Output: } $\theta^*_{\rightleftarrows}$}
\end{algorithmic}

%\vspace{0.2cm}

\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\caption{A brief depiction of the training pipeline.}\label{fig:alg_wiki}
\vspace{-1em}
\end{figure}
